Overcoming Barriers to Skill Injection in Language Modeling: Case Study in Arithmetic

Through their transfer learning abilities, highly-parameterized large pre-trained language models have dominated the NLP landscape for a multitude of downstream language tasks. Though linguistically proficient, the inability of these models to incorporate the learning of non-linguistic entities (numerals and arithmetic reasoning) limits their usage for tasks that require numeric comprehension or strict mathematical reasoning. However, as we illustrate in this paper, building a general purpose language model that also happens to be proficient in mathematical reasoning is not as straight-forward as training it on a numeric dataset. In this work, we develop a novel framework that enables language models to be mathematically proficient while retaining their linguistic prowess. Specifically, we offer information-theoretic interventions to overcome the catastrophic forgetting of linguistic skills that occurs while injecting non-linguistic skills into language models.

==> rough.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Example-Image}
        \caption[Network2]%
        {{\small Network 1}}    
        \label{fig:mean and std of net14}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{Example-Image}
        \caption[]%
        {{\small Network 2}}    
        \label{fig:mean and std of net24}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Example-Image}
        \caption[]%
        {{\small Network 3}}    
        \label{fig:mean and std of net34}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Example-Image}
        \caption[]%
        {{\small Network 4}}    
        \label{fig:mean and std of net44}
    \end{subfigure}
    \caption[ The average and standard deviation of critical parameters ]
    {\small The average and standard deviation of critical parameters: Region R4} 
    \label{fig:mean and std of nets}
\end{figure*}


\begin{table}[h]
\centering
\footnotesize
\caption{\footnotesize{Caption for Table.}}
\label{table:main}
\begin{tabular}{l|l|lllll}
\hline
                   & \textit{ln} RMSE          & CoLA                       & MNLI                                & MRPC                        & SST-2                      & STS-B                      \\ \hline
Base               & $3.5367_{0.0000}$            & \multicolumn{1}{c}{$\textbf{0.4827}_{0.0000}$} & \multicolumn{1}{c}{$\textbf{0.8074}_{0.0000}$} & \multicolumn{1}{c}{$\textbf{0.8797}_{0.0000}$} & \multicolumn{1}{c}{$\textbf{0.8967}_{0.0000}$} & \multicolumn{1}{c}{$\textbf{0.8740}_{0.0000}$} \\
Base + Arithmetics & $0.4443_{0.0112}$ & $0.0000_{0.0000}$                        & $0.3553_{0.0012}$                   & $0.7524_{0.0009}$           & $0.8761_{0.0032}$          & $0.3998_{0.0799}$          \\
Ours               & $\textbf{0.4360}_{0.0169}$ & $0.4193_{0.0003}$          & $0.7951_{0.0041}$                   & $0.8570_{0.0000}$              & $0.8962_{0.0089}$          & $0.8626_{0.0053}$          \\ \hline
\end{tabular}
\end{table}

\begin{enumerate}
    \item \note{Talk about Kirkpatrick paper, add necessary background and formulae.}
    \item \note{Define formulation of proposed model i.e., DistillBERT + ewc Addition (Follow GenBERT problem formulation structure.)}
    \item \note{Add a dataset description section.}
    \item \note{In an Experimental Setup Section, talk about specifics of training: Epochs, Architecture, selection of $\lambda$ etc.}
\end{enumerate}
